Emotion pattern detection on facial videos using functional statistics

There is an increasing scientific interest in automatically analysing and understanding human behavior, with particular reference to the evolution of facial expressions and the recognition of the corresponding emotions. In this paper we propose a technique based on Functional ANOVA to extract significant patterns of face muscles movements, in order to identify the emotions expressed by actors in recorded videos. We determine if there are time-related differences on expressions among emotional groups by using a functional F-test. Such results are the first step towards the construction of a reliable automatic emotion recognition system

==> 3_oldmethods.tex <==
\section{Methods}


%In this analysis, functional data objects are constructed from the AUs time series, by specifying a set of basis functions and a set of coefficients defining a linear combination of these basis functions. The B-spline basis is used for non-periodic functions. B-spline basis functions are polynomial segments jointed end-to-end at argument values called knots, breaks or join points, and they have the advantages of very fast computation and great flexibility \cite{ramsay2004functional} \cite{ramsay2020package}. 

%By decomposing functions via a functional principal component analysis (FPCA), we can investigate the dominant modes of variation of functional data. FPCA represents functional data in the most parsimonious way, in the sense that when using a fixed number of basis functions, the eigenfunction basis explains more variation than any other basis expansion \cite{happ2018multivariate}.


%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%

%\url{https://hal.archives-ouvertes.fr/hal-00943745/document}

Let $\Omega$ be a population space of action units and $s_n = \{\omega_1, \omega_2,\dots, \omega_n\}$ be a random sample set of size $n$ drawn from $\Omega$. Assume $\mathbf{Y}$ is a random variable defined on $\Omega$ associating to $\omega \in \Omega$ and containing a set of $D$ variates ($D=17$ in this case), each defined on the finite interval $[0, T], 0 < T < +\infty$, i.e
$\mathbf{Y}(\omega) = {(Y_{\omega,1}(t), \dots,Y_{\omega,d}(t), \dots, Y_{\omega,D}(t)), t \in [0, T]}.$
The observation of $\mathbf{Y}$ on the sample $s_n$ provides the set ${\mathbf{Y}(\omega_1),\dots, \mathbf{Y}(\omega_n)}$ of multivariate curves, called multivariate functional data. From $n$ curves, one can be interested in optimal
representation of curves in a reduced dimensional function space. In order to address in a formal way, we further assume that for $\mathbf{Y} = (\mathbf{Y}_1,\dots, \mathbf{Y}_d, \dots, \mathbf{Y}_D)^T$, $\mathbf{Y}_d$, $d = 1, \dots, D$ is $L_2([0, T])$-valued random variable and $\mathbf{Y}$ is a $D$ dimensional $L_2$ continuous stochastic process.
%$$\lim\limits_{h\to 0} \mathbb{E} [||\mathbf{Y}(t+h) - \mathbf{Y}(t)||^2] = \lim\limits_{h\to 0}\int_0^T\sum\limits_{k=1}^K \mathbb{E}  [(\mathbf{Y}_k(t+h) - \mathbf{Y}_k(t))^2] dt = 0.$$


The mean functions of $Y_d$ and $\mathbf{Y}$ are
\begin{equation*}
    \mu_d = \mu_d(t) = \mathbb{E}[\mathbf{Y}_d(t)], t \in [0, T], \text{ and } \mathbf{\mu} = (\mu_1, \dots,\mu_d, \dots,\mu_D)^T = \mathbb{E[\mathbf{Y}]}.
\end{equation*}
The covariance operator of $\mathbf{Y}$ is defined as an integral operator $C$ with kernel
$$C(t,s) = \mathbb{E}[(\mathbf{Y}(t)-\mathbf{\mu}(t))\otimes (\mathbf{Y}(s)-\mathbf{\mu}(s))], \forall t,s \in [0, T], $$

where $\otimes$ is the tensor product on $\mathbb{R}^D$. Thus, $C(t,s)$ is a $D \times D$ matrix with elements
$$C(t,s)[i,j] = Cov(\mathbf{Y}_i(t),\mathbf{Y}_j(s)), i,j = 1, \dots,D.$$

Under the hypothesis of $L_2$-continuity, $C$ is an Hilbert-Schmidt operator, i.e., it is compact and self-adjoint.

\subsection{Functional Principal Component Analysis}
\label{sec:methoed - alignment}


The spectral analysis of $C$ provides a countable set of positive eigenvalues $\{\eta_{j, j \geq 1}\}$ associated to an orthonormal basis of eigen-functions $\{\mathbf{f}_{j,j\geq 1}\}$, $\mathbf{f}_j = (f_{j,1},\dots, f_{j,D})$:
$$C\mathbf{f}_j = \eta_j\mathbf{f}_j,$$
with $\lambda_1 \geq \lambda_2 \geq \dots$ and $\langle \mathbf{f}_i,\mathbf{f}_j \rangle _{\{L_2([0,T])\}^D} = \delta_{i,j}$ with $\delta_{i,j} = 1$ if $i=j$, otherwise $\delta_{i,j} =0$. We define the principal component $C_j$ of $\mathbf{Y}$, zero-mean random variable, as the projections of  $\mathbf{Y}$ on the $j$th eigenfunction of $C$:

\begin{equation}
    C_j = \int_0^T \langle \mathbf{Y}(t) - \mathbf{\mu}(t),  \mathbf{f}_j (t) \rangle dt = \int_0^T \sum\limits_{d=1}^D(Y_d(t) - \mu_d(t))f_{j,d}(t)dt
\end{equation}

This means that $\mathbf{Y}(t)$ varies around the mean function with random amplitude variations in the directions of $\{ \mathbf{f}_j \}_{j \geq 1}$. Thus the following Karhunen-Loeve expansion holds

\begin{equation}
    \mathbf{Y}(t) = \mathbf{\mu}(t) + \sum\limits_{j \geq 1}C_j\mathbf{f}_j (t),\ \  Y_d(t) = \mu_d(t) + \sum\limits_{j \geq 1}C_j\mathbf{f}_{j,d} (t),
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Functional Registration}
\label{sec:methoed - alignment}

As mentioned before, it is essential to align the unregistered chronological timeline of action units curves into a common registered internal timeline that follows the same pronunciation speed, to control the influence of the speech itself and to study the influence sourced from the emotions. Therefore, we need to isolate the phase variability of the action unit curves, at the same time, keeping the amplitude-phase unchanged to maintain the information of the intensity level of the action units. 

The phase variation is normally represented by a random change of time scale, which is mostly a non-linear transformation. 
We use the warping functions $T_i: [0,T] \rightarrow [0,T], i = 1, \dots, n$, assuming that they are increasing functions independent of amplitude variation. They map unregistered chronological time $t_i^*$ to registered internal time $t$ such that $T_i^{-1}(t_i^*) = t$ and with $E[T_i(t)] = t$. The observed time-warped curves 
$$\tilde{Y}_{i,d}(t) = Y_{i,d}(T_i^{-1}(t_i^*)) = \mu_{d}(T_i^{-1}(t_i^*)) + \sum\limits_{j \geq 1} C_j\mathbf{f}_{j,d} (T_i^{-1}(t_i^*)).$$

%Therefore, we have $$E[ \tilde{Y}(x) | T ] = \mu(T^{-1}(x)) = \tilde{\mu}(x), $$ $$Cov\{ \tilde{Y}(x), \tilde{Y}(y) \} = E[\kappa( T^{-1}(x), T^{-1}(y) )] + Cov\{ \tilde{\mu}(x), \tilde{\mu}(y) \}. $$ Here we can already notice that the functions $\phi_n(T_i^{-1}(x))$ are no longer the eigenfunctions of the covariation $Cov\{ \tilde{Y}(x), \tilde{Y}(y) \}$. Thus it proves that the estimation would be distorted if we ignore the phase variation term.


%The literature is rich of proper methods to do this, and a more in-depth review would be beyond the scope of this report. We follow the principal components based registration method provided by the R package "registr" \cite{wrobel2018register}. 

%On the time grid $\{t_m\}_{m=1}^M$, the discrete values of the curve $\tilt{Y}_{i,k}(t)$ is $$ \tilde{Y}_{i,k,m} = Y_{i,k}(t_m) + \epsilon_{i,k,m},\ \  i = 1,\dots,n, m = 1,\dots,M.$$ 

We follow the principal components based registration method with a generative process, where codes are available in the R package "registr" \cite{wrobel2018register}. Briefly speaking, we consider probabilistic FPCA in EM algorithm process, to calculate iteratively the mean and covariance of $\mathbf{Y}(t)$ conditioned on the current inverse warping functions that map the observed curves to the templates, and then estimate the inverse warping functions $T_i^{-1}(t_i^*)$ by maximizing the log likelihood of the probability function of $\mathbf{Y}(t)$ given the current estimates of mean and covariance. In this way, the registered internal timeline obtained carries the same amplitude information, capable for the task of analyzing action units among different videos.



\subsection{Functional Linear Model}

  
The registered curves of 17 action units among neutral and other 7 emotions (calm, happy, sad, angry, fearful, surprise, and disgust) are available for us to represent the curves as registered smooth functions. The question to approach here is whether there exist patterns which could describe the variations of action units attributable significantly to one emotion. 

In functional linear modelling setting, let $Y_{d,k,g}(t), t \in [0,T]$ be the evolution of action unit $d\in \{1,\dots,D\}$ in the video $k \in \{1,\dots,K\}$ for emotion $g\in \{1,\dots,7\}$. For the sake of simplicity, we denote $y_{k,g}(t) = Y_{d,k,g}(t)$ under the situation for focusing on a fixed action unit $d$. We can assume that
\begin{equation}
y_{k,g}(t) = \mu_0(t) + \alpha_{g}(t) + \epsilon_{k,g}(t),
\label{flm:indiv}
\end{equation}
where $\mu_0(t)$ is the grand mean function due to the sentence, and therefore indicates the average engagement degree across all emotions. The term $\alpha_{g}(t)$ is the specific effect on action unit $d$ of emotion $g$. $\epsilon_{k,g}(t)$ represents unexplained variation with zero mean, specific to the $k$-th video within emotion group $g$. To be able to identify them uniquely, we require that they satisfy the constraint
$\sum\limits_{g=1}^7 \alpha_{g}(t) = 0, \forall t.$


We can define a $8K \times 8$ design matrix $\mathbf{Z}$ for this model, with one row for each action unit curve, as follows. Use the label $(k, g)$ for the row corresponding to video $k$ in emotion $g$. The first $K$ rows represent the videos in neutral case, while every $K$ rows below contains videos with one specific emotion in order. We write $z_{k,g}$ for the $8$-vector whose transpose is the $(k, g)$ row of $\mathbf{Z}$.

%We can then define a corresponding set of five regression functions $\beta_j$ by setting $\beta_1 = \mu$, $\beta_2 = \alpha_1$, and so on to $\beta_8 = \alpha7$,so that the functional vector $\mathbf{\beta} =  (\mu, \alpha_1, \alpha_2, \alpha_3, \dots, \alpha_7)$. 

Equation \ref{flm:indiv} can be written with the matrix formulation:
$\mathbf{y}=\mathbf{Z}\mathbf{\beta} + \mathbf{\epsilon},$ with
$$\mathbf{y}=\begin{bmatrix}
y_{1,0}(t) \\
\vdots \\
y_{K,0}(t) \\
y_{1,1}(t) \\
\vdots \\
y_{K,1}(t) \\
y_{1,2}(t) \\
\vdots \\
y_{K,2}(t) \\
 \\
 y_{1,7}(t) \\
\vdots \\
y_{K,7}(t)
\end{bmatrix},
\mathbf{Z}=
\begin{bmatrix}
1 & 0 & 0 & 0 &   \cdots & 0 & 0 \\
\vdots & \vdots   & \vdots & \vdots & \cdots & \vdots & \vdots \\
1 & 0 & 0 & 0 &   \cdots & 0 & 0 \\
1 & 1 & 0 & 0 &   \cdots & 0 & 0 \\ 
\vdots & \vdots  & \vdots & \vdots & \cdots & \vdots & \vdots \\
1 & 1 & 0 & 0 &   \cdots & 0 & 0 \\ 
1 & 0 & 1 & 0 &   \cdots & 0 & 0 \\ 
\vdots & \vdots &   \vdots & \vdots & \cdots & \vdots & \vdots \\
1 & 0 & 1 & 0 &   \cdots & 0 & 0 \\ 
  &   &   &     & \cdots &   &  \\
1 & 0 & 0 & 0 &   \cdots & 0 & 1 \\ 
\vdots & \vdots   & \vdots & \vdots & \cdots & \vdots & \vdots \\
1 & 0 & 0 & 0 &   \cdots & 0 & 1 
\end{bmatrix},
\mathbf{\beta} = \begin{bmatrix}
\mu_0(t) \\
\alpha_1(t)\\
\vdots \\
\alpha_7(t)
\end{bmatrix} = \begin{bmatrix}
\beta_1(t) \\
\beta_2(t)\\
\vdots \\
\beta_8(t)
\end{bmatrix},
$$
where $\mathbf{\beta}$ is defined as the corresponding set of eight regression functions for neutral and emotional types, and $\mathbf{\epsilon}$ is the matrix of noise with the same dimension of $\mathbf{y}$. In these terms, Equation \ref{flm:indiv} has the equivalent formulation:
 
\begin{equation}
y_{k,g}(t)  = \sum\limits_{j=1}^8  z_{k,g,j} \beta_j(t)+\epsilon_{k,g}(t) = \langle z_{k,g},\mathbf{\beta}(t) \rangle + \epsilon_{k,g}(t).
\end{equation}



\iffalse
or, more compactly in matrix notation,
\begin{equation}
\mathbf{Y} = \mathbf{Z} \mathbf{\beta} + \mathbf{\epsilon},
\end{equation}
\fi

%where $\mathbf{Y}$ is the vector containing the 35 temperature functions, $\mathbf{\epsilon}$ is a vector of 35 residual functions, and $\mathbf{\beta}$ is the 5-vector of parameter functions. The design matrix $\mathbf{Z}$ has exactly the same structure as for the corresponding univariate or multivariate one-way analysis of variance. The only way in which (9.4) differs from the corresponding equations in standard elementary textbooks on the general linear model is that the parameter $\mathbf{\beta}$, and hence the predicted observations $\mathbf{Z}\mathbf{\beta}$, are vectors of functions rather than vectors of numbers.

%The standard least squares criterion would say that $\mathbf{\beta}$ should be chosen to minimize the residual sum of squares, which can be written $\|\mathbf{Y} - \mathbf{Z}\mathbf{\beta}\|^2$ in vector notation. To extend the least squares principle to the functional case, we need only reinterpret the squared norm in an appropriate way. The quantity $\mathbf{Y} - \mathbf{Z}\mathbf{\beta}$ is now a vector of functions. The individual components of $\mathbf{Z}\mathbf{\beta}$ are the individual predictors $<z_{(k,g)},\mathbf{\beta}(t)>$, and so 




To estimate the parameters we use the functional least squares fitting criterion with the norm compiled in $L_2([0,T])$ space 
\begin{equation}
   \hat{\mathbf{\beta}}(t) = \arg \min\limits_{\mathbf{\beta}} \sum\limits_{g=1}^8 \sum\limits_{k=1}^K \int_0^T [y_{k,g} (t) - \langle z_{k,g},\mathbf{\beta}(t) \rangle]^2 dt,
\end{equation}
subject to the constraint 
$0 = \sum\limits_{i = 1}^7 \alpha_i(t) = \sum\limits_{j = 2}^8 \beta_j(t) = \mathbf{L}\mathbf{\beta}(t), \forall t$ with $\mathbf{L} = [0,1,1,\dots,1]$



%Regularization involves attaching a penalty term to the basic squared-error fitting criterion:
%\begin{equation}
%    LMSSE_\lambda(B) =  \|Y - ZB \|^2 + \lambda * PEN(B).
%\end{equation}
%The purpose of the penalty term PEN(B) is to require that the estimated value of B not only yields a good fit in the sense of small $\|Y - ZB\|^2$, but also that some aspect of B captured in the function PEN is kept under control. 




\subsection{Functional Analysis of Variance (FANOVA)}


In estimating emotion effects, we have characterized the action units' patterns for videos in each emotion. We may wish to move on and not only confirm that the total emotion-specific effect $\alpha_g$ is nonzero, but also investigate whether this effect is substantial at a specific time $t$. We can make a hypothesis by assuming that we want to test whether for emotion $\tilde{g}$ at time $t$, action unit $d$ is not significantly different from the "neutral" mean function $\mu_0(t)$:
$ H_0: \alpha_{\tilde{g}}(t) = 0.$



%error sum of squares functions LMSSE, squared correlation functions RSQ, and F-ratio functions FRATIO. It is the dependence of these quantities on t that makes the procedure different from the standard multivariate case.


As in the multivariate linear model, the primary source of information in investigating the importance of the zone effects $\alpha_g$ is the sum of squares of residuals function:

\begin{equation}
    SSE(t) = \sum\limits_{k,g} [y_{k,g}(t) - (\mathbf{Z}\hat{\mathbf{\beta}})_{k,g}(t)]^2.
\end{equation}


The sum of squares of residuals function with estimated $\hat{\mathbf{\beta}}_{H_0}$ under assumption $H_0$ is:
\begin{equation}
    SSH_0(t) = \sum\limits_{k,g, g\neq \tilde{g}} [y_{k,g}(t) - (\mathbf{Z}\hat{\mathbf{\beta}}_{H_0})_{k,g} (t)]^2.
\end{equation}


We can compute the functional analogues of the mean square for error function $MSE(t)$:
$MSE(t) = \frac{SSE(t)}{\text{df(error)}},$
where $\text{df(error)}$ is the degrees of freedom for error, or the sample size $N$ less the number of mathematically independent functions $\beta_q$ in the model. In this problem, the zero sum restriction on the climate zone effects $\alpha_g$ implies that there are four degrees of freedom lost to the model, or $\text{df(error)} = 31$. 

Similarly, the mean square for error function under assumption $H_0$ is the difference between $SSH_0(t)$ and $SSE(t)$, divided by the difference between the degrees of freedom for error for the two models:
$MSR(t) = \frac{SSH_0(t) - SSE(t)}{df(model)}.$

Finally, we can compute the functions FRATIO:
\begin{equation*}
    FRATIO(t) = \frac{MSR(t)}{MSE(t)} \sim\limits_{H_0} \mathcal{F}_{1, size},
\end{equation*}
and reject $H_0$ if $FRATIO(t) > c_{1-\alpha}$, where $c_{1-\alpha}$ is the critial value at level $1-\alpha$ of $\mathcal{F}_{1, size}$.


